Radiative Decays of the Spin-$\nicefrac{3}{2}$ to Spin-$\nicefrac{1}{2}$ Doubly Heavy Baryons in QCD

The spin-$\nicefrac{3}{2}$ to spin-$\nicefrac{1}{2}$ doubly heavy baryon transition magnetic dipole $G_M$ and electric quadrupole $G_E$ formfactors are calculated in the framework of light cone sum rules method. Moreover, the decay widths of corresponding radiative transitions are estimated. Obtained results of magnetic dipole moments $G_M$ and decay widths are compared with the results present in the literature.

==> references.tex <==
\bibliographystyle{ieeetr}
\bibliography{ref}
